Online Variant of Parcel Allocation in Last-mile Delivery

We investigate the problem of last-mile delivery, where a large pool of citizen crowd-workers are hired to perform a variety of location-specific urban logistics parcel delivering tasks. Current approaches focus on offline scenarios, where all the spatio temporal information of parcels and workers are given. However, the offline scenarios can be impractical since parcels and workers appear dynamically in real applications, and their information is unknown in advance. In this paper, in order to solve the shortcomings of the offline setting, we first formalize the online parcel allocation in last-mile delivery problem, where all parcels were put in pop-stations in advance, while workers arrive dynamically. Then we propose an algorithm which provides theoretical guarantee for the parcel allocation in last-mile delivery. Finally, we verify the effectiveness and efficiency of the proposed method through extensive experiments on real and synthetic datasets.

==> ______yudian <==
１．您提的这些问题确实是我之前没理清楚的。
第一，我之前确实是思考得不够，导致问题定义看起来很别扭。今天跟童老师讨论了一下，他也觉得我的问题定义在现实生活中是较难找到应用场景的。因此我改为：

首先我还是做最后一公里派送的online版本，但是我的目标函数是使得平台收益最大化。其次平台给每个工人有相应的最大预算(budget)，再次工人没有capacity。也就是说工人做得越多，会赚的越多，但是在一天之内做得再多，也拿不到额外费用。

就类似于咱们在玩游戏，用户每玩一局游戏都得到一些经验值，但是一天之内玩到一定的次数，经验值就不会再增加了。（比如三国杀）你可以反驳我说，没有费用我为什么还要去派送快递？有些人也不一定需要奖励才会去做某些事情的，比如有时候只是顺路，给捎带一下什么的。我觉得这个问题也不是说不过去。

那我的问题就变为一个分配问题，就是平台把parcels分配给工人就完事了，就不需要再考虑其他的。比如说什么送达时间，送达时间是worker自己跟客户之间商量的，或者路线什么的，路线可以是由worker直接问客户走那条路最近。

那我的问题本质就是一个parcel的分配问题。不是planning问题。



２．每个parcel针对每个工人都有不同的费用。这就像您说的由配送速度，交通工具类型决定。



３.如果真要写，这个例子得重新写一下。

4.topk team,这文章？我没看到这文章呢，我是直接拿模板来说的。是dawei gao的那篇吗？

５．修饰后一句的归约。有一部分是一样的，但是有一部分是不一样.不一样的地点是在parcels到workers的边的流，因为我的文章是求平台的效益最大，而在转变的为min-cost　flow时，边上的流值不能直接写效益的值，而是我对这个值做了转变（U'）。

６．您说的是图几？横坐标是|c|的意思是改变worker的capacity,这个capacity服从1~6的随机分布。
其中图４的a~c,横坐标的是|c|确实是我放错了，应该是\mu. 谢谢指正。


7.这个我可能确实是没表达清楚。



８．图5的a~c中的横坐标表示的是用户从1万增加到5万，因此这里的横坐标：|P| X 10^-4 = 横坐标的值，而不是10^4.在图5的a中的纵坐标utility X 10^-5 = 纵坐标的值，utility = 纵坐标的值 X 10 ^5. 因此这里的数值没有错。其实还有一种写法，横坐标：|P|*(10^4)，这种写法也是对的。加括号和不加括号是有区别的。


In addition, each worker can quoted price for each parcel according to its distance and weight. However, crowdsourcing platform in order to pursuit the maximum benefit that they will give a reasonable parcel allocation to reduce the additional expenditure. In particular, each parcel has different price for different workers　according to the speed of workers' delivery or the type of vehicle.








